Fine-tuning multilingual language models in Twitter/X sentiment analysis: a study on Eastern-European V4 languages

The aspect-based sentiment analysis (ABSA) is a standard NLP task with numerous approaches and benchmarks, where large language models (LLM) represent the current state-of-the-art. We focus on ABSA subtasks based on Twitter/X data in underrepresented languages. On such narrow tasks, small tuned language models can often outperform universal large ones, providing available and cheap solutions. We fine-tune several LLMs (BERT, BERTweet, Llama2, Llama3, Mistral) for classification of sentiment towards Russia and Ukraine in the context of the ongoing military conflict. The training/testing dataset was obtained from the academic API from Twitter/X during 2023, narrowed to the languages of the V4 countries (Czech Republic, Slovakia, Poland, Hungary). Then we measure their performance under a variety of settings including translations, sentiment targets, in-context learning and more, using GPT4 as a reference model. We document several interesting phenomena demonstrating, among others, that some models are much better fine-tunable on multilingual Twitter tasks than others, and that they can reach the SOTA level with a very small training set. Finally we identify combinations of settings providing the best results.

==> unused/podklady.tex <==
Russia hit Ukarine with rockets and missiles
Ukraine hit Russia with rockets and missiles
Putin is a dictator
Zelensky is a dictator
They bombed Donbass
Ukraians only money

ChatGPT
Sure, let's break down the sentiment analysis for each aspect in these sentences:

Aspect: Russia's actions towards Ukraine

Sentence: "Russia hit Ukraine with rockets and missiles"
Sentiment: Negative
Confidence: 0.7
Aspect: Ukraine's actions towards Russia

Sentence: "Ukraine hit Russia with rockets and missiles"
Sentiment: Negative
Confidence: 0.8
Aspect: Vladimir Putin

Sentence: "Putin is a dictator"
Sentiment: Negative
Confidence: 0.9
Aspect: Volodymyr Zelensky

Sentence: "Zelensky is a dictator"
Sentiment: Neutral to Negative (It's essential to note that calling Zelensky a dictator might not be accurate or fair, so the sentiment might be negative depending on the perspective, but it could also be seen as neutral if it's recognized as misinformation or hyperbole.)
Confidence: 0.6
Aspect: Those involved in bombing Donbass (unclear from the sentence who 'they' refers to)

Sentence: "They bombed Donbass"
Sentiment: Negative (assuming 'they' refers to one of the parties involved in the conflict)
Confidence: 0.7
Aspect: Ukrainians and their financial situation

Sentence: "Ukrainians only money"
Sentiment: Unclear (the sentence seems incomplete or unclear in meaning)
Confidence: N/A
User
do it once more always provide the sentiment towards Russia and Ukraine for each sentence
ChatGPT
Sure, let's analyze the sentiment towards Russia and Ukraine in each sentence:

Sentence: "Russia hit Ukraine with rockets and missiles"

Sentiment towards Russia: Negative
Sentiment towards Ukraine: Negative
Confidence: Russia - 0.7, Ukraine - 0.8
Sentence: "Ukraine hit Russia with rockets and missiles"

Sentiment towards Russia: Negative
Sentiment towards Ukraine: Negative
Confidence: Russia - 0.8, Ukraine - 0.7
Sentence: "Putin is a dictator"

Sentiment towards Russia: Neutral to Negative
Sentiment towards Ukraine: N/A
Confidence: Russia - 0.9
Sentence: "Zelensky is a dictator"

Sentiment towards Russia: N/A
Sentiment towards Ukraine: Neutral to Negative
Confidence: Ukraine - 0.6
Sentence: "They bombed Donbass"

Sentiment towards Russia: Negative (if 'they' refers to Russia or Russian-backed forces)
Sentiment towards Ukraine: Negative (if 'they' refers to Ukrainian forces)
Confidence: Russia - 0.7, Ukraine - 0.7
Sentence: "Ukrainians only money"

Sentiment towards Russia: N/A
Sentiment towards Ukraine: Unclear
Confidence: N/A


---------------------------------


Absolutely! Here's the sentiment analysis for each sentence, considering both Russia and Ukraine:

Sentence: "Russia hit Ukraine with rockets and missiles"

Russia Sentiment (Aspect): Negative (Aggressive action)
Confidence: 0.8
Ukraine Sentiment (Aspect): Negative (Being attacked)
Confidence: 0.9
Sentence: "Ukraine hit Russia with rockets and missiles"

Russia Sentiment (Aspect): Negative (Being attacked)
Confidence: 0.8
Ukraine Sentiment (Aspect): Positive (Potential defense) - Confidence adjusted based on context.
Confidence: 0.7 (Lower confidence due to the lack of explicit justification for the attack in the sentence, but higher than a neutral response considering the ongoing conflict).
Sentence: "Putin is a dictator"

Russia Sentiment (Aspect): Negative (Dictatorial leadership)
Confidence: 0.9
Ukraine Sentiment (Aspect): Neutral
Confidence: 0.5
Sentence: "Zelensky is a dictator"

Russia Sentiment (Aspect): Neutral
Confidence: 0.5
Ukraine Sentiment (Aspect): Negative (Dictatorial leadership)
Confidence: 0.8
Sentence: "They bombed Donbass"

Russia Sentiment (Aspect): Positive (Potentially - depends on perspective on the conflict)
Confidence: 0.6 (Lower confidence due to the complex situation in Donbass)
Ukraine Sentiment (Aspect): Negative (Region being bombed)
Confidence: 0.8
Sentence: "Ukrainians only money"

Russia Sentiment (Aspect): Neutral
Confidence: 0.5
Ukraine Sentiment (Aspect): Negative (Stereotype)
Confidence: 0.7


\subsection{A sentiment and it's aspect}
Gemini conversation:
Aspect-Based Sentiment Analysis:

**Sentence:** "Ukraine hit Russia with rockets and missiles"

**Analysis:**

* **Russia:** Negative Sentiment (Score: 0.8, Confidence: 0.7)
    * "Hit" and "rockets/missiles" imply an attack, leading to a negative sentiment for Russia.
    * Confidence is moderate (0.7) because the sentence doesn't explicitly mention the morality of the attack. 
* **Ukraine:** Mixed Sentiment (Score: 0.3, Confidence: 0.5)
    * The sentence is neutral towards Ukraine's action itself ("hit"). 
    * However, considering the ongoing conflict, there could be an implicit positive sentiment for Ukraine defending itself (not reflected in the score).
    * Confidence is low (0.5) due to the sentence's neutrality and lack of context about the justification for the attack.

**Limitations:**

* This is a simplified analysis based on a single sentence. More context is needed for a more comprehensive understanding.
* Sentiment analysis tools may not perfectly capture the nuances of human language and intent.

Overall, the sentence suggests a negative event for Russia (being attacked) and a mixed sentiment for Ukraine (acting but justification unclear). The confidence scores reflect the limitations of analyzing a single sentence without broader context.

\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Sentence} & \multicolumn{2}{|c|}{\textbf{Russia Sentiment}} & \multicolumn{2}{|c|}{\textbf{Ukraine Sentiment}} \\ \cline{2-5}
 & Aspect & Confidence  & Aspect & Confidence \\ \hline
Russia hit Ukraine with rockets and missiles  & Aggressive action  & 0.8  & Being attacked  & 0.9  \\ \hline
Ukraine hit Russia with rockets and missiles  & Being attacked  & 0.8  & Potential defense  & 0.7  \\ \hline
Putin is a dictator  & Dictatorial leadership  & 0.9  & Neutral  & 0.5 \\ \hline
Zelensky is a dictator  & Neutral  & 0.5  & Dictatorial leadership  & 0.8  \\ \hline
They bombed Donbass  & Potentially positive (depends on perspective)  & 0.6  & Region being bombed  & 0.8  \\ \hline
Ukrainians only money & Neutral  & 0.5  & Stereotype  & 0.7 \\ \hline
\end{tabular}


\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{Sentence} & \multicolumn{2}{c|}{Sentiment} & \multirow{2}{*}{Confidence} \\ \cline{2-3}
 & Russia & Ukraine &  \\ \hline
Russia hit Ukraine with rockets and missiles & Negative & Negative & Russia: 0.7, Ukraine: 0.8 \\ \hline
Ukraine hit Russia with rockets and missiles & Negative & Negative & Russia: 0.8, Ukraine: 0.7 \\ \hline
Putin is a dictator & Neutral to Negative & N/A & Russia: 0.9 \\ \hline
Zelensky is a dictator & N/A & Neutral to Negative & Ukraine: 0.6 \\ \hline
They bombed Donbass & Negative & Negative & Russia: 0.7, Ukraine: 0.7 \\ \hline
Ukrainians only money & N/A & Unclear & N/A \\ \hline
\end{tabular}
\caption{Sentiment Analysis Results}
\label{tab:sentiment}
\end{table}


Tohle az do jineho clanku

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|l|@{}}
\toprule
\textbf{Text for ABSA / Model (R,U)}         & \textbf{LLama} & \textbf{Mistral} & \textbf{Bert} & \textbf{Bertweet} & \textbf{GPT 3.5} & \textbf{GPT 4} & \textbf{Gemini} & \textbf{GPT2} & \textbf{LLama Z} & \textbf{MistralZ} & \textbf{BertZ} \\ \midrule
                                             &                &                  &               &                   &                  &                &                 &               &                  &                   &                \\ \midrule
Russia hit Ukraine with rockets and missiles &                &                  &               &                   & N0.7, N0.8       &                &                 &               &                  &                   &                \\ \midrule
Ukraine hit Russia with rockets and missiles &                &                  &               &                   & N0.7, N0.8       &                &                 &               &                  &                   &                \\ \midrule
Putin is a dictator                          &                &                  &               &                   &                  &                &                 &               &                  &                   &                \\ \midrule
Zelensky is a dictator                       &                &                  &               &                   &                  &                &                 &               &                  &                   &                \\ \midrule
They bombed Donbass                          &                &                  &               &                   &                  &                &                 &               &                  &                   &                \\ \midrule
Ukrainians only want more money                &                &                  &               &                   &                  &                &                 &               &                  &                   &                \\ \bottomrule
\end{tabular}
\end{table}



First take only the Czech(+Slovak) dataset, make a multidimensional scoreboard:

\begin{itemize}
    \item DIM 1 various models: Llama2, BERT, BERTweet, Mistral, 
    \item DIM 2 on reference model (GPT? Mistral?) various translations: Google Translate (JEN ANOTACE - POMOC), Helsinki, DeepL
    \red{Only DeepL and Helsinki}
    \item DIM 3 take the best translation, compare: reference model with translation / reference multilingual model without translation
    \item DIM 4: the best of the previous one, influence of fine.tuning, dataset selection methodology (reference tweets), etc.
    \item DIM 5: best of the previous, prompt engineering, try 0-shot, few shot, instruction \red{We do not do instructions}
\end{itemize}
Subsequently, take the best achieved variant and perform for Hungarian and Polish\\
Compare sentiments or other aspects of differences between languages.\\
Incorporate a comparison with SetFit-ABSA?

========================================


We took a sample of sentences from tweets, translated them in English and queried different model to get the sentiment score towards specific aspect.



Complex tweet - simple sentiment
Complex tweet - ABSA
Simple "product" sentiment vs. train of thoughts

Ukraine is at war - is this positive or negative?
Ukraine bombs Russia - is this neutral, or negative towards UA
Russia bombs Ukraine - is this neutral, or negative towards RU
Sors is buying land in Ukraine - is this neutral, or is this negative effect, or is this and insult to UA
Putin should be destroyed - negative towards Ru
General XYZ should be destroyed - without context we can not 

==> unused/tmp.tex <==
The set of experiments is meant rather as a proof of concept and the creation of a basic methodology to track this (sentiment) in general - that means having data that is worked with using different models and we evaluate the results - model performance, experience etc.

\begin{itemize}
    \item Metrics - basic metrics, confusion matrix, possibly inference time, RAM demand...
    \item Description of processing of the entire data package
    \item Results
    \item 
\end{itemize}

\textbf{Maximalistic scheme of experiments:
}
\medskip

First take only the Czech(+Slovak) dataset, make a multidimensional scoreboard:

\begin{itemize}
    \item DIM 1 various models: Llama2, Bert, Mistral \red{We do not have Bert}
    \item DIM 2 on reference model (GPT? Mistral?) various translations: Google Translate, Helsinki, DeepL
    \red{Only DeepL and Helsinki}
    \item DIM 3 take the best translation, compare: reference model with translation / reference multilingual model without translation
    \item DIM 4: the best of the previous one, influence of fine.tuning, dataset selection methodology (reference tweets), etc.
    \item DIM 5: best of the previous, prompt engineering, try 0-shot, few shot, instruction \red{We do not do instructions}
\end{itemize}
Subsequently, take the best achieved variant and perform for Hungarian and Polish\\
Compare sentiments or other aspects of differences between languages.\\
Incorporate a comparison with SetFit-ABSA?

========================================






\subsection{Results}



5 & ukraine & hu & mistralai & origin & reduced & positive & 0.8598130841121495 & 0.86 & 0.8431372549019608 & 0.8514851485148515 \\
6 & ukraine & hu & meta-llama & origin & reduced & negative & 0.8598130841121495 & 0.8596491228070176 & 0.875 & 0.8672566371681416 \\
7 & ukraine & hu & meta-llama & origin & reduced & positive & 0.8598130841121495 & 0.86 & 0.8431372549019608 & 0.8514851485148515 \\
8 & russia & hu & mistralai & origin & ref & negative & 0.8543689320388349 & 0.9056603773584906 & 0.8275862068965517 & 0.8648648648648648 \\
9 & russia & hu & mistralai & origin & ref & positive & 0.8543689320388349 & 0.8 & 0.8888888888888888 & 0.8421052631578948 \\
\end{longtable}\hline \end{tabularx}


\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
\toprule
 & target & lang & model & translator & tw & type & acc & precision & recall & f1 \\ \midrule
\midrule
0 & russia & hu & mistralai & origin & reduced & negative & 0.883495145631068 & 0.859375 & 0.9482758620689655 & 0.9016393442622951 \\ \midrule
1 & russia & hu & mistralai & origin & reduced & positive & 0.883495145631068 & 0.9230769230769231 & 0.8 & 0.8571428571428571 \\ \midrule
2 & russia & pl & meta-llama & origin & reduced & negative & 0.8627450980392157 & 0.9111111111111111 & 0.803921568627451 & 0.8541666666666666 \\ \midrule
3 & russia & pl & meta-llama & origin & reduced & positive & 0.8627450980392157 & 0.8245614035087719 & 0.9215686274509803 & 0.8703703703703703 \\ \midrule
4 & ukraine & hu & mistralai & origin & reduced & negative & 0.8598130841121495 & 0.8596491228070176 & 0.875 & 0.8672566371681416 \\ \midrule
5 & ukraine & hu & mistralai & origin & reduced & positive & 0.8598130841121495 & 0.86 & 0.8431372549019608 & 0.8514851485148515 \\ \midrule
6 & ukraine & hu & meta-llama & origin & reduced & negative & 0.8598130841121495 & 0.8596491228070176 & 0.875 & 0.8672566371681416 \\ \midrule
7 & ukraine & hu & meta-llama & origin & reduced & positive & 0.8598130841121495 & 0.86 & 0.8431372549019608 & 0.8514851485148515 \\ \midrule
8 & russia & hu & mistralai & origin & ref & negative & 0.8543689320388349 & 0.9056603773584906 & 0.8275862068965517 & 0.8648648648648648 \\ \midrule
9 & russia & hu & mistralai & origin & ref & positive & 0.8543689320388349 & 0.8 & 0.8888888888888888 & 0.8421052631578948 \\ \midrule
\bottomrule
\end{tabular}



\begin{table}[]
\begin{tabular}{lccll}
\hline

\multicolumn{1}{|c|}{\textbf{Specific Model}} & \multicolumn{1}{c|}{\textbf{Accuracy}} & \multicolumn{1}{c|}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{Support}} \\ \hline

\multicolumn{1}{|c|}{LLama-DeepL-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\end{tabular}
\caption{Assessment for a specific model after initial training on a spcific dataset and specific language subset}
\end{table}



\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Tweets / Language}                  & Czech (CS) & Slovak (SK) & Polish (PL) & Hungarian (HG) \\ \hline
\textbf{Tweets total}                       &            &             &             &                \\ \hline
\textbf{Training tweets}                    &            &             &             &                \\ \hline
\textbf{Training tweets positive (Ukraine)} &            &             &             &                \\ \hline
\textbf{Training tweets negative (Ukraine)} &            &             &             &                \\ \hline
\textbf{Training tweets neutral (Ukraine)}  &            &             &             &                \\ \hline
\end{tabular}
\textbf{\caption{Dataset and sub datasets with their size used for training of models. Ukraine dataset.}}
\end{table}

\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Tweets / Language}                  & Czech (CS) & Slovak (SK) & Polish (PL) & Hungarian (HG) \\ \hline
\textbf{Tweets total}                       &            &             &             &                \\ \hline
\textbf{Training tweets}                    &            &             &             &                \\ \hline
\textbf{Training tweets positive (Russian)} &            &             &             &                \\ \hline
\textbf{Training tweets negative (Russian)} &            &             &             &                \\ \hline
\textbf{Training tweets neutral (Russian)}  &            &             &             &                \\ \hline
\end{tabular}
\textbf{\caption{Dataset and sub datasets with their size used for training of models. Russian dataset.}}
\end{table}


\begin{table}[]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Specific model}         & \textbf{Model} & \textbf{Transaltor (if any)} & \textbf{Training set focus} & \textbf{Language of training set} \\ \hline

\textbf{LLama-DeepL-ukraine-cs} & \textbf{LLama} & \textbf{DeepL} & \textbf{ukraine} & \textbf{cs} \\ \hline
LLama-DeepL-ukraine-sk          & LLama          & DeepL          & ukraine          & sk          \\ \hline
LLama-DeepL-ukraine-pl          & LLama          & DeepL          & ukraine          & pl          \\ \hline
LLama-DeepL-ukraine-hg          & LLama          & DeepL          & ukraine          & hg          \\ \hline
LLama-DeepL-russia-cs           & LLama          & DeepL          & russia           & cs          \\ \hline
LLama-DeepL-russia-sk           & LLama          & DeepL          & russia           & sk          \\ \hline
LLama-DeepL-russia-pl           & LLama          & DeepL          & russia           & pl          \\ \hline
LLama-DeepL-russia-hg           & LLama          & DeepL          & russia           & hg          \\ \hline
LLama-Helsinki-ukraine-cs       & LLama          & Helsinki       & ukraine          & cs          \\ \hline
LLama-Helsinki-ukraine-sk       & LLama          & Helsinki       & ukraine          & sk          \\ \hline
LLama-Helsinki-ukraine-pl       & LLama          & Helsinki       & ukraine          & pl          \\ \hline
LLama-Helsinki-ukraine-hg       & LLama          & Helsinki       & ukraine          & hg          \\ \hline
LLama-Helsinki-russia-cs        & LLama          & Helsinki       & russia           & cs          \\ \hline
LLama-Helsinki-russia-sk        & LLama          & Helsinki       & russia           & sk          \\ \hline
LLama-Helsinki-russia-pl        & LLama          & Helsinki       & russia           & pl          \\ \hline
LLama-Helsinki-russia-hg        & LLama          & Helsinki       & russia           & hg          \\ \hline
LLama-None-ukraine-cs           & LLama          & None           & ukraine          & cs          \\ \hline
LLama-None-ukraine-sk           & LLama          & None           & ukraine          & sk          \\ \hline
LLama-None-ukraine-pl           & LLama          & None           & ukraine          & pl          \\ \hline
LLama-None-ukraine-hg           & LLama          & None           & ukraine          & hg          \\ \hline
LLama-None-russia-cs            & LLama          & None           & russia           & cs          \\ \hline
LLama-None-russia-sk            & LLama          & None           & russia           & sk          \\ \hline
LLama-None-russia-pl            & LLama          & None           & russia           & pl          \\ \hline
LLama-None-russia-hg            & LLama          & None           & russia           & hg          \\ \hline
Mistral-DeepL-ukraine-cs        & Mistral        & DeepL          & ukraine          & cs          \\ \hline
Mistral-DeepL-ukraine-sk        & Mistral        & DeepL          & ukraine          & sk          \\ \hline
Mistral-DeepL-ukraine-pl        & Mistral        & DeepL          & ukraine          & pl          \\ \hline
Mistral-DeepL-ukraine-hg        & Mistral        & DeepL          & ukraine          & hg          \\ \hline
Mistral-DeepL-russia-cs         & Mistral        & DeepL          & russia           & cs          \\ \hline
Mistral-DeepL-russia-sk         & Mistral        & DeepL          & russia           & sk          \\ \hline
Mistral-DeepL-russia-pl         & Mistral        & DeepL          & russia           & pl          \\ \hline
Mistral-DeepL-russia-hg         & Mistral        & DeepL          & russia           & hg          \\ \hline
Mistral-Helsinki-ukraine-cs     & Mistral        & Helsinki       & ukraine          & cs          \\ \hline
Mistral-Helsinki-ukraine-sk     & Mistral        & Helsinki       & ukraine          & sk          \\ \hline
Mistral-Helsinki-ukraine-pl     & Mistral        & Helsinki       & ukraine          & pl          \\ \hline 
Mistral-Helsinki-ukraine-hg     & Mistral        & Helsinki       & ukraine          & hg          \\ \hline
Mistral-Helsinki-russia-cs      & Mistral        & Helsinki       & russia           & cs          \\ \hline
Mistral-Helsinki-russia-sk      & Mistral        & Helsinki       & russia           & sk          \\ \hline
Mistral-Helsinki-russia-pl      & Mistral        & Helsinki       & russia           & pl          \\ \hline
Mistral-Helsinki-russia-hg      & Mistral        & Helsinki       & russia           & hg          \\ \hline
Mistral-None-ukraine-cs         & Mistral        & None           & ukraine          & cs          \\ \hline
Mistral-None-ukraine-sk         & Mistral        & None           & ukraine          & sk          \\ \hline
Mistral-None-ukraine-pl         & Mistral        & None           & ukraine          & pl          \\ \hline
Mistral-None-ukraine-hg         & Mistral        & None           & ukraine          & hg          \\ \hline
Mistral-None-russia-cs          & Mistral        & None           & russia           & cs          \\ \hline
Mistral-None-russia-sk          & Mistral        & None           & russia           & sk          \\ \hline
Mistral-None-russia-pl          & Mistral        & None           & russia           & pl          \\ \hline
Mistral-None-russia-hg          & Mistral        & None           & russia           & hg         
\end{tabular}
\caption{Overview of specific models which were trained on data and specific translation or without translation.}
\end{table}

\begin{table}[]
\begin{tabular}{lccll}
\hline

\multicolumn{1}{|c|}{\textbf{Specific Model}} & \multicolumn{1}{c|}{\textbf{Negative - Russia}} & \multicolumn{1}{c|}{\textbf{Posotive - Russia}} & \multicolumn{1}{c|}{\textbf{Negative - Ukraine}} & \multicolumn{1}{c|}{\textbf{Positive - Ukrine}} \\ \hline

\multicolumn{1}{|c|}{LLama-DeepL-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-DeepL-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-Helsinki-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{LLama-None-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-DeepL-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-Helsinki-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-ukraine-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-cs}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-sk}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-pl}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\multicolumn{1}{|c|}{Mistral-None-russia-hg}
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
&
\multicolumn{1}{|c|}{ }
\\ \hline
\end{tabular}
\caption{Results of the annotation of the dataset with specific trained models and their results (positive, negative sentiment towards Russia and Ukraine)}
\end{table}


\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{Dataset} & \textbf{Pro Ukrainian} & \textbf{Anti Ukrainian} & \textbf{Pro Russian} & \textbf{Anti Russian} \\ \hline
                    &                       &                      &                      &                      &                       \\ \hline
                    &                       &                      &                      &                      &                       \\ \hline
                    &                       &                      &                      &                      &                       \\ \hline
\end{tabular}
\caption{Sentiment assessment with a specific model on a specific dataset}
\end{table}

MARTIN: PLEASE ADD FURTHER TABLES HERE

\subsection{Discussion}
\label{sec_discussion}

\textbf{Evaluation of the effectiveness of individual solutions and the definition of the one that appears to be the best}

Which metric is the most important from our point of view and for our situation. What model configuration appeared to be the best and by what percentage to the worst, what was the worst.

\medskip
\textbf{Sentiment, context of knowledge, effect of situation} 
Complex tweet - simple sentiment
Complex tweet - ABSA
Simple "product" senttiment vs. train of thoughts

Ukraine is at war - is this positive or negative?
Ukraine bombs Russia - is this neutral, or negative towards UA
Russia bombs Ukraine - is this neutral, or negative towards RU
Sors is buying land in Ukraine - is this neutral, or is this negative effect, or is this and insult to UA
Putin should be destroyed - negative towards Ru
General XYZ should be destroyed - without context we can not 



\textbf{Regional context of tweets} 
Complex twwet - simple sentiment
Complex tweet - ABSA

Ukraine is at war - is this positive or negative?
Ukraine bombs Russia - is this neutral, or negative towards UA
Russia bombs Ukraine - is this neutral, or negative towards RU
Sors is buying land in Ukraine - is this neutral, or is this negative effect, or is this and insult to UA

\medskip
\textbf{Situations and models that showed a strange error rate} 

- what and where it was happening
Was there something that really surprised us, if so what was it, what did the tweet look like and what was the behavior of the model, or on the contrary what method was special on its own.

\medskip
\textbf{Impact of translation into English, or use of the model over the native text (cz, sk, pl, mg)}

Why we think it's good to translate things into English, how each translation differed and what was the impact on the observed efficiency.

\medskip
\textbf{The importance of the number of parameters on the effectiveness of the model}
\red{We do not do this in our experiment}

Is the significance of the number of parameters so massive, how much does it differ in percentages in the variations performed and why do we think this is so.

\medskip
\textbf{Models and current data
}
\red{We should do a specific experiment - focusing on these words in the tweets and in the LLM, to find out the reality, what does the model know}
The models don't have to have actual actual data - such as the name and definition of a person, how can we pass these things - for example, that the president is not Poroshenko, but Zelensky.

\medskip
\textbf{Difficulty in implementing the solution - preparing a conversation or something automated}
\red{Do we really have a conversation?}

Do we generally have to prepare things by hand, or can it be automated, done completely without thinking, or is there a better approach. That doesn't mean I'm talking about how I prepared things.

\medskip
\textbf{The importance of asking questions and prompt tuning
}
\red{We do not have a real conversation, just a question and and answer}
This turns out to be an effective approach. Here we would write about what we tried and how it affected us. Related to this is the creation of conversations as a more effective way of performing annotation.

\textbf{Relevance of results: } we are on a limited range of data, so the values are not very informative, because we would need to process a substantially larger sample of the monitored social network. So we rather focus on the methods of working with ABSA and compare them, and let the actual result of what we measured as a kind of bonus, with a discussion here whether it would make sense if these things were monitored on a large scale.

Napady:

Pseudo labbeling - iterovat nad datasety a pak tim labelovat a sledovat vykon toho, jak to funguje.


